A New Simulation Metric to Determine Safe Environments and Controllers for Systems with Unknown Dynamics

We consider the problem of extracting safe environments and controllers for reach-avoid objectives for systems with known state and control spaces, but unknown dynamics. In a given environment, a common approach is to synthesize a controller from an abstraction or a model of the system (potentially learned from data). However, in many situations, the relationship between the dynamics of the model and the \textit{actual system} is not known; and hence it is difficult to provide safety guarantees for the system. In such cases, the Standard Simulation Metric (SSM), defined as the worst-case norm distance between the model and the system output trajectories, can be used to modify a reach-avoid specification for the system into a more stringent specification for the abstraction. Nevertheless, the obtained distance, and hence the modified specification, can be quite conservative. This limits the set of environments for which a safe controller can be obtained. We propose SPEC, a specification-centric simulation metric, which overcomes these limitations by computing the distance using only the trajectories that violate the specification for the system. We show that modifying a reach-avoid specification with SPEC allows us to synthesize a safe controller for a larger set of environments compared to SSM. We also propose a probabilistic method to compute SPEC for a general class of systems. Case studies using simulators for quadrotors and autonomous cars illustrate the advantages of the proposed metric for determining safe environment sets and controllers.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> sections/alternate_repr.tex <==
\subsection{Alternate Interpretation}
\shromona{Need to integrate with problem statement section}
An alternative way to interpret the distance metric $\distMetricOld$ and $\distMetricNew$ is through the size of the set $\Env_{\spec}(\dist)$, defined as 
%
\begin{align} \label{eqn:alt_int:env_sets}
\Env_{\spec}(\dist) = & \{\env \in \Env: \exists \ctrlseq \in \controlspace, \traj_{\abs}(\cdot; \state_0, \ctrlseq) \models \spec(\env; \dist) \rightarrow \traj_{\sys}(\cdot; \state_0, \ctrlseq) \models \spec(\env) \}, \\
\Env_{\spec} = & \{\env \in \Env: \exists \ctrlseq \in \controlspace, \traj_{\abs}(\cdot; \state_0, \ctrlseq) \models \spec(\env), \traj_{\sys}(\cdot; \state_0, \ctrlseq) \models \spec(\env) \}. \nonumber
\end{align}
%












==> sections/compare_distmetrics.tex <==
\subsection{Comparing distance metrics}\label{sec:compare_dist}
We have already discussed how the simulation metric in~\eqref{eqn:sim_metric:naive} provides an overly conservative distance metric, $\distMetricOld$.

Before we arrive at our proposed simulation metric~\eqref{eqn:sim_metric:proposed}, $\distMetricNew$; we consider two other distance metrics,
\begin{enumerate}
    \item $\distMetricIntOne$ defined as:
        \begin{equation}
        \label{eqn:sim_metric:naive2}
        \distMetricIntOne = \max_{\env \in \Env} \max_{u \in \controlspace_{\spec(\env)}} \|\traj_{\sys}(\cdot; \state_0, \ctrlseq) - \traj_{\abs}(\cdot; \state_0, \ctrlseq) \|_{\infty}, 
        \end{equation}
        Where we compute the $\infty$ norm between the $\sys$ and $\abs$ trajectories when the $\traj_{\abs}(\cdot) \models \spec(\env)$. 
        We do not consider $\traj_{\abs}(\cdot) \not\models \spec(\env)$ since, such controllers would not be helpful in the context of the $\sys$.
    \item $\distMetricIntTwo$ defined as:
        \begin{equation}
        \label{eqn:sim_metric:naive3}
        \distMetricIntTwo = \max_{\env \in \Env} \max_{u \in \controlspace_{\spec(\env)}} \|\traj_{\sys}(\cdot; \state_0, \ctrlseq) - \traj_{\abs}(\cdot; \state_0, \ctrlseq) \|_{\infty} \cdot \mathbbm{1}_{\left(\traj_{\sys}(\cdot) \not \models \spec(\env)\right)}, 
        \end{equation}
        Where we compute the $\infty$ norm between the $\sys$ and $\abs$ trajectories when the $\traj_{\abs}(\cdot) \models \spec(\env)$ and $\traj_{\sys}(\cdot) \not\models \spec(\env)$. Here we further restrict to controllers where $\traj_{\sys}(\cdot) \not\models \spec(\env)$. This is because if a $\ctrlseq$ is able to correctly control the $\sys$; the distance between the resulting trajectories should not be considered. 
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[scale=0.40]{figures/compare_dist.pdf}
    \caption{Comparing $\distMetricIntOne$, $\distMetricIntTwo$ and $\distMetricNew$}
    \label{fig:comparing_dists}
\end{figure}

In Figure~\ref{fig:comparing_dists}, we how the different metrics are computer. Let us consider the trajectories generated by two pairs of $(\env_1, \ctrlseq_1), (\env_2, \ctrlseq_2) \in  \domain$. 
The first pair, $(\env_1, \ctrlseq_1)$,  generates $\traj_{\abs}$ ($\traj_{\sys}$) shown in dotted (solid) purple line. Here, since $\traj_{\abs}(\cdot) \models \spec(\env)$, it contributes to~\eqref{eqn:sim_metric:naive2}; and hence $\distMetricIntOne > 0$. However, since $\traj_{\sys}(\cdot) \models \spec(\env)$, it does not contribute to~\eqref{eqn:sim_metric:naive3} and~\eqref{eqn:sim_metric:proposed}; and $\distMetricIntTwo = \distMetricNew = 0$. 
The second pair, $(\env_2, \ctrlseq_2)$ generates $\traj_{\abs}$ ($\traj_{\sys}$) shown in dotted (solid) red line. Again since $\traj_{\abs}(\cdot) \models \spec(\env)$, we have $\distMetricIntOne > 0$. Here, $\traj_{\sys}(\cdot) \not\models \spec(\env)$; and we have $\distMetricIntTwo > \distMetricNew > 0$. In fact $\distMetricIntTwo$ considers the infinity norm between the trajectories which is always than the~\eqref{eqn:dist_fn:proposed}; and we have $\distMetricIntTwo > \distMetricNew$. 
If $\distMetricIntOne$ is greater for $(\env_1, \ctrlseq_1)$, we would have $\distMetricIntOne > \distMetricIntTwo > \distMetricNew > 0$.

Each of the distance metrics introduced here ensures that $\Env_{\spec}(\dist) \subset \Env_{\spec}$. This is guaranteed for $\distMetricNew$ because of Proposition~\ref{prop:main_result_1} and we have shown that $\distMetricOld, \distMetricIntOne, \distMetricIntTwo > \distMetricNew$. 

\shromona{Should we mention something about uniformly contracting the expanding the $\reachSet$ and $\avoidSet$}

==> sections/old_problem_formulation.tex <==
\section{Notation and Definitions}
\label{sec:not_defn}
We define by $\Env := (\initStates, \avoidSets, \reachSets, \envParams)$ the set of all environmental scenarios, where we want to synthesize a controller for the system. $\Env$ is a composition of $\initStates$ the set of all initial states of the system, $\avoidSets$ the set of all avoid scenarios, $\reachSets$ the set of all reach scenarios and $\envParams$ the set of all other environment parameters that affect the synthesis, such as disturbances, lighting conditions in a vision-based controller, etc. 
Therefore, a particular environment scenario $\env \in \Env$ is a four-tuple, $(\state_0, \avoidSet(\cdot), \reachSet(\cdot), \envParam)$, where $\state_0$ is the initial state of the system, $\avoidSet(\cdot)$ and $\reachSet(\cdot)$ are (potentially time varying) avoid and the reach sets respectively; and $\envParam$ is the environment parameters. 
One could consider the $\state_0, \avoidSet(\cdot), \reachSet(\cdot)$ in $\envParam$, however, we define them separately to highlight their importance in our framework. 
For brevity, we summarize the key notations in the following table: %Table~\ref{tab:notation}
%
\begin{center} \label{tab:notation}
 \begin{tabular}{|c|c|c|} 
 \hline
 Notation & Represents & Set element\\  
 \hline
 $\Env$ & Environment set & $\env$
 \\
 $\initStates$ & Set of initial states & $\state_0$ 
 \\
 $\avoidSets$ & Set of avoid sets & $\avoidSet(\cdot)$ 
 \\ 
 $\reachSets$ & Set of reach sets & $\reachSet(\cdot)$
 \\
 $\envParams$ & Environment parameters &  $\envParam$
 \\
 $\timeHorizon$ & Time horizon & $\time$
 \\
 $\abs$ & The system abstraction & - 
  \\
 $\sys$ & The system & -
 \\
 $\traj(\time)$ & Trajectory at time $t$ & -
 \\
 $\spec$ & Reach-avoid specification & -
 \\
 $\controlspace$ & Control space & $\ctrlseq$
 \\
 \hline
\end{tabular}
\end{center}
%

We represent by $\sys$ and $\abs$, the system and an associated abstraction for $\sys$.
%For each $\env \in \Env$, we are interested in synthesizing a controller, $\ctrlseq_{\env}(\cdot)$, for the system, $\sys$; such that the resulting finite time horizon, $\timeHorizon = \{0, 1, \ldots, \horizon\}$, trajectory starting from the initial state $\state_0$, satisfies the given reach-avoid specification.
We consider trajectories defined on a finite time horizon $\timeHorizon = \{0, 1, \ldots, \horizon\}$.
For a given $\env\in \Env$ and an associated controller $\ctrlseq_{\env}(\cdot)$, we say a trajectory $\traj(\cdot; \state_0, \ctrlseq_{\env})$ starting from the initial state $\state_0$ satisfies a reach-avoid specification $\spec(\env)$ (equivalently $\traj(\cdot; \state_0, \ctrlseq_{\env}) \models \spec(\env)$) if
%
\begin{equation} \label{eqn:problem:spec}
%  \traj(0; \ctrlseq_{\env}) = \state_0 ~\text{and}~ 
 \forall t \in \timeHorizon \; \traj(t; \state_0, \ctrlseq_{\env}) \notin \avoidSet(t), \traj(t; \state_0, \ctrlseq_{\env}) \in \reachSet(t).
\end{equation}
%
For the ease of notation, we drop $\ctrlseq_{\env}$ and $\state_0$ from the trajectory arguments wherever convenient. The trajectory generated by the $\sys$ ($\abs$) is represented as $\traj_{\sys}$ ($\traj_{\abs}$).

%Further, we define $\forall t \in \timeHorizon$,
%\begin{equation}
%    \label{eqn:spec:state}
%    \spec_t(\env) = \{\traj(t): \traj(t) \notin \avoidSet(t) \wedge \traj(t) \in \reachSet(t)\}
%\end{equation}
%i.e., $\spec_t(\env)$ is the set of all states that are safe at time $t$.

%We also say $\traj(t) \models \spec_t(\env)$ if $\traj(t) \in \spec_t(\env)$. 
%Therefore, $\traj(\cdot) \models \spec(\env)$ if and only if $\forall t \in \timeHorizon, %\traj(t) \models \spec_t(\env)$. 

$\spec(\env)$ is a trace property, i.e., the satisfaction of the specification depends on a trace of $\sys$.
More succinctly, we can define $\spec(\env)$ as the set of all trajectories that satisfy the reach-avoid specification, i.e.,
\begin{equation}
    \label{eqn:spec:unmodified}
    \spec(\env) :=\{\traj(\cdot): \traj(t) \notin \avoidSet(t) \wedge \traj(t) \in \reachSet(t) \; \forall t \in \timeHorizon\}
\end{equation}
Hence, a $\traj(\cdot)\models \spec(\env)$ if and only if $\traj(\cdot)\in \spec(\env)$.
% \SBnote{We might have to change these definitions a little bit to account for the environmental parameters that do not affect the reach or the avoid sets, but still affect the trajectory we take. For example, in the lane keeping example, the position of the other car/lighting conditions affect the occlusion which in turn affect the controller and ultimately the system trajectory. But the car's position does not affect the avoid set/reach set as such. }
In our definition we allow a time-varying $\reachSet(\cdot)$ and $\avoidSet(\cdot)$. 
If the sets are not time varying, we can replace $\reachSet(\cdot)$ ($\avoidSet(\cdot)$) by the stationary $\reachSet$ ($\avoidSet$).
Similarly, if there is no avoid or reach set at a particular time, we can use $A(t) = \emptyset$ and $R(t) = \mathcal{X}$, where $\mathcal{X}$ is the state space of the system.

Typically, one synthesizes controllers using a particular control policy $\Pi$, e.g., linear feedback controllers, which limits the set of generated controllers. 
We represent this set of controllers by, $\controlspace_{\Pi} \subseteq \controlspace$. 

\section{Problem Formulation}
\label{sec:prob_form}
We are interested in verifying that the $\sys$ can safely operate in environments $\Env$. Formally, we would like to prove, 
\begin{equation}
\label{eqn:verif_guarantee}
    \forall \env \in \Env \, \exists \ctrlseq_{\env} \in \controlspace_{\Pi}\; \traj_{\sys}(\cdot; \state_0, \ctrlseq_{\env}) \models \spec_{\env} 
\end{equation}
%\SBnote{Explain what happens when there is no avoid set or no reach set at a particular time.}
Formally verifying~\eqref{eqn:verif_guarantee} is difficult for several reasons,
\begin{enumerate}
    \item For a given control policy, \eqref{eqn:verif_guarantee} may not hold $\forall \env \in \Env$.
    \item In general, we may not have access to the dynamics model of the $\sys$ (i.e., $\sys$ is a black-box). We assume that it is available as an oracle that we can query (such as a simulator).
    \item We generally rely on an abstraction $\abs$ (potentially learnt from data) to design $\controlspace_{\Pi}$.
\end{enumerate}

Our goal in this work is to verify~\eqref{eqn:verif_guarantee} (if true) or find the largest set, where, 
\begin{equation}
\label{eqn:env_assump}
    \{\env \in \Env: \exists \ctrlseq \in \controlspace_{\Pi}\,, \traj_{\sys}(\cdot; \state_0, \ctrlseq) \models  \spec(\env) \}
\end{equation}
we can provide verification guarantees. 

However, to find~\eqref{eqn:env_assump}, we must be able to generate controllers for $\sys$. 
When a dynamics model of $\sys$ or its conservative abstraction is known, several methods have been studied in literature to verify~\eqref{eqn:verif_guarantee} or find~\eqref{eqn:env_assump} for reach-avoid problems~\cite{tomlin1998conflict, mitsch2013provably, tomlin2000game}.
%\shromona{Have to clean up the below discussion to bring in the notion of bisimulation or simulation metric}
However, we are interested in the scenario when a dynamics model for $\sys$ is not available--only a system abstraction, $\abs$, is available. 
Here, $\abs$ may not necessarily be a conservative approximation of $\sys$ and the bounds between $\abs$ and $\sys$ are not available beforehand.
This might happen for example when $\abs$ is obtained through data-driven methods, such as using function approximators like Neural networks, where the model quality bounds that can be used for verification purposes are generally not available. We assume that $\abs$ and $\sys$ have the same state and control domain.

The abstraction $\abs$, has two purposes in our framework: (1) to synthesize controllers for $\sys$ (synthesis); and (2) provide safety guarantees on the synthesized controllers on the $\sys$ (verification). Specifically, we would like to find the  set of environments, $\Env_{\spec}$, where we synthesize safe controllers for $\abs$ using the policy $\Pi$, which are also safe for the $\sys$. Formally, 
\begin{equation}
    \label{eqn:env_assum_with_model}
    \tilde{\Env}_{\spec} := \{\env \in \Env: \exists \ctrlseq \in \controlspace_{\Pi}\,, \traj_{\abs}(\cdot; \state_0, \ctrlseq)  \models \spec(\env)\,, \traj_{\sys}(\cdot; \state_0, \ctrlseq) \models \spec(\env) \}
\end{equation}
$\tilde{\Env}_{\spec}$ is the set of environments where there exists at least one controller that is safe for both the $\abs$ and $\sys$. It is the set of all environmental scenarios for which it is possible to synthesize a safe controller for the system using the abstraction. This is \textbf{largest} set for which $\abs$ can be used to synthesize safe controllers for $\sys$. For $\tilde{\Env}_{\spec}$ we cannot synthesize controllers for $\sys$ using the $\abs$!

We are interested in finding the largest $\tilde{\Env}_{\spec}$ in~\eqref{eqn:env_assum_with_model}. In the finite sample regime, if for an $\env \in \tilde{\Env}_{\spec}$, we find a controller $\ctrlseq$ such that $\traj_{\abs} \models \spec_{\env}$, we cannot comment if $\traj_{\sys}$ is safe. Hence, we cannot provide any safety guarantees based on $\abs$ alone.
Hence, we would have to exhaustively search the entire space $\controlspace_{\Pi}$ for each $\env \in \tilde{\Env}_{\spec}$ to provide meaningful guarantees using $\abs$. This makes the computation of $\tilde{\Env}_{\spec}$ in-feasible in practical settings.

A computationally less expensive set to compute is finding the set of environment where if the the controller is safe for $\abs$ it is also safe for $\sys$, i.e., 
\begin{equation}
    \Env_{\spec} = \{\env \in \Env: \forall \ctrlseq \in \controlspace_{\Pi}\,, \traj_{\abs}(\cdot) \models \spec_{\env} \rightarrow \traj_{\sys}(\cdot) \models \spec_{\env} \}
\end{equation}
Within $\Env_{\spec}$, $\abs$ can be used instead of $\sys$ to both synthesize controllers and verify $\traj_{\sys}(\cdot) \models \spec_{\env}$.


==> sections/quadrotor_old.tex <==
\subsection{Safe Altitude Control for Quadrotor}
\label{sec:quadrotor}
In this simulation, we demonstrate the safety-preserving performance of our distance metric through a quadrotor simulation.
We use the reach-avoid setting described in~\cite{fisac2017general}, where the authors are interested in controlling the altitude of a quadrotor in an indoor setting while ensuring that it does not go too close to the ceiling or the floor.

A dynamic model of quadrotor vertical flight can be written as:
\begin{align} \label{eqn:quad:model}
    z(t+1) = & z(t) + Tv_z(t) \nonumber \\
    v_z(t+1) = & v_z(t) + T(ku(t) + g),
\end{align}
where $z$ is the vehicle's attitude, $v_z$ is its vertical velocity and $u$ is the commanded average thrust.
The gravitational acceleration is $g = -9.8 m/s^2$ and the discretization step $T$ is 0.01.
The control input $u(t)$ is bounded to $[0, 1]$.
We are interested in designing a controller for $\sys$ that ensures safety over a horizon of 100 timesteps. 
In particular, we have $\initStates = \{(z, v_z): 0.5 \leq z \leq 2.5,  -3\leq v_z \leq 3\}$, $\avoidSets = \{\avoidSet(\cdot)\}, \reachSets =\mathbb{R}^2$ and $\envParams = \emptyset$. 
The avoid set at any time $\time$ is given as $\avoidSet(t) = \{(z, v_z) \in \mathbb{R}^2: 0.5m \leq z(t) \leq 2.5m\}$.

We again assume that the dynamics in \eqref{eqn:quad:model} are unknown and only the dynamics of an abstraction are known.
Our goal is to obtain the best possible conservative approximation of $\Env_{\spec}$ using $\abs$ and a distance bound between $\sys$ and $\abs$.
Let's consider an abstraction with the same dynamics as in \eqref{eqn:quad:model}, except that, $k_{\abs}$, the value of parameter $k$ in the abstraction dynamics is different.
In particular, we consider two scenarios: $k_{\abs} < k$ and $k_{\abs} > k$.
For each scenario, we compute four different distance bounds between $\sys$ and $\abs$: $\distMetricOld, \distMetricIntOne, \distMetricIntTwo$ and $\distMetricNew$, as defined in \eqref{eqn:sim_metric:naive}, \eqref{eqn:sim_metric:naive2}, \eqref{eqn:sim_metric:naive3} and \eqref{eqn:sim_metric:proposed} respectively. 
For fairness, for $\distMetricOld, \distMetricIntOne$ and $\distMetricIntTwo$, we measure the distance only between the $z$ states as only $z$ affects the avoid specification, rather than measuring the distance between all the states.
% $\distMetricNew$ is already defined to measure the distance only between the relevant states (so $g(\state) = z$ in this case).
We use Algorithm \ref{alg:solution} with the corresponding distance functions to compute these bounds.

The space of controllers $\controlspace_{\Pi}$ is given by all possible control sequences over the time horizon (i.e., $\controlspace_{\Pi} = \controlspace$.) 
For computing $\controlspace_{\spec(\env)}$, we use the Level Set Toolbox~\cite{mitchell2008flexible} that gives us both the set of initial states from which there exist a controller that will keep the abstraction trajectory outside the avoid set at all times (i.e., the set $\Env_{\spec}(0)$, which is also called the reachable set), as well as the corresponding least restrictive controller.
In particular, we can apply any control when the abstraction trajectory is inside the reachable set and the safety-preserving control (given by the toolbox) when the trajectory is near the boundary of the reachable set. 
For computation of the distance bounds, we sample a random controller sequence according to this safety-preserving control law.
If any initial state lies outside the reachable set, then it is also guaranteed that $\controlspace_{\spec(\env)}=\emptyset$ so we do not need to do any rejection sampling in this case.

When $k_{\abs} < k$, the abstraction has strictly less control authority compared to the system.
Thus any controller that satisfies the specification for $\abs$ must also satisfy the specification for $\sys$. 
Consequently, we should have $\distMetricNew = 0$ (by Proposition \ref{prop:main_result_3}.)
Indeed, we computed the distance bound using Algorithm \ref{alg:solution} and the obtained numbers are $\distMetricOld=0.30, \distMetricIntOne=0.50, \distMetricIntTwo=0, \distMetricNew=0$.
As expected, $\distMetricNew=0$.
Note that even though $\distMetricOld$ is smaller than $\distMetricIntOne$ in this case, it may not be particularly useful in synthesizing a safe controller for the system.
This is because $\distMetricOld$ computed using a scenario optimization approach ensures that a safe controller designed on the abstraction for the modified specification is also safe for the system with high probability, only when this controller is \textit{randomly} selected from the set $\controlspace$.
However, a random controller selected from $\controlspace$ is unlikely to satisfy the modified specification for the abstraction itself, and thus we cannot say anything about the system either.
In contrast, for the other three distance metrics, we sample a controller from the set $\controlspace_{\spec(\env)}$ during the scenario optimization.
Therefore, during the controller synthesis process too, we \textit{randomly} select a controller from the set $\controlspace_{\spec(\env; \dist)}$, which is guaranteed to be safe on both the abstraction and the system with high probability.
%
\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{./figures/reach_sets_cons}
    \caption{Different reachable sets when the quadrotor abstraction is conservative.
    The distance metrics $\distMetricNew$ and $\distMetricIntTwo$ only considers the distance between trajectories that violates the specification on the system and satisfies it on the abstraction, leading to a less conservative estimate of the distance.}
    \label{fig:quad_example:reach_sets_conservative}
    % \vspace{-1.7em}
\end{figure}
%

For illustration purposes, we also compute the reachable sets $\Env_{\spec}(\distMetricIntOne)$, $\Env_{\spec}(\distMetricIntTwo)$ and $\Env_{\spec}(\distMetricNew)$, by augmenting the avoid set by the corresponding distance bounds and recomputing the reachable sets using the Level Set Toolbox.
As shown in Figure \ref{fig:quad_example:reach_sets_conservative}, $\Env_{\spec}(0)$ is contained within $\Env_{\spec}^{\sys}$, which is the set of all states for which it is possible to synthesize a safe controller for the system (computed using the system dynamics).
Thus, any controller that is safe on the abstraction is also safe on the system, i.e., $\Env_{\spec}(0) = \Env_{\spec}$.
Since $\distMetricIntTwo=\distMetricNew=0$ in this case, we are able to recover $\Env_{\spec}$ exactly, as shown by the black and the magenta contours. 
On the other hand, $\Env_{\spec}(\distMetricIntOne)$ (the green contour) is a significantly smaller subset of $\Env_{\spec}$, and hence, we can synthesize a safe controller only for a much smaller set of environments.
Also note that $\Env_{\spec}(\distMetricIntTwo) = \Env_{\spec}(\distMetricNew)$ in this case. 
In fact, it can be shown that is the case whenever $\abs$ is a conservative model of $\sys$. 
However, when that is not the case, $\Env_{\spec}(\distMetricIntTwo)$ can be quite conservative too, as illustrated next.
%
\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{./figures/reach_sets_opt}
    \caption{Different reachable sets when the quadrotor abstraction is overly optimistic.
    The distance metric $\distMetricNew$ achieves a far less conservative under-approximation of $\Env_{\spec}$ compared to the other distance metrics.}
    \label{fig:quad_example:reach_sets_optimistic}
    % \vspace{-1.7em}
\end{figure}
%

When $k_{\abs} > k$, the system has strictly less control authority compared to the abstraction.
Consequently, there might exist some environments for which it is possible to synthesize a safe controller for the abstraction, but the same controller when deployed on the system might lead to an unsafe behavior.
Therefore, $\Env_{\spec}^{\sys} = \Env_{\spec}$.
We again compute the distance bound using Algorithm \ref{alg:solution} and the obtained numbers are $\distMetricOld=0.30, \distMetricIntOne=0.49, \distMetricIntTwo=0.49, \distMetricNew=0.1$.
The corresponding reachable sets are shown in Figure \ref{fig:quad_example:reach_sets_optimistic}.
Even though we start with an overly optimistic abstraction, all the distance metrics is able to compute an under approximation of $\Env_{\spec}$; however, the sets estimated by 
$\distMetricIntOne$ and $\distMetricIntTwo$ are overly conservative.
$\distMetricNew$ on the other hand is still able to recover $\Env_{\spec}$ to a very good accuracy.
% , indicating that it is sufficient to consider the minimum distance across time steps at which the specification is violated rather than maximum distance across all time steps.

\SBnote{At the end of the section, explain how obtaining the distance bound as proposed can be the first step in a lot of safe learning/Fastrack kinds of works that require a conservative model of the system.}

\shromona{Have discussion on $\abs$ being a conservative approximation of $\sys$}



% Starting from an initial state, the system safety specification is given as \SBnote{Check with Shromona on the formal way of writing a specification}
% \begin{equation} \label{eqn:quad:spec}
% \spec := \forall t \in \{0, 1, \ldots, H\}, 0.5m \leq z(t) \leq 2.5m
% \end{equation}

% The goal is to find the viability kernel $\viableset_{\sys}$ which is the set of all initial states such that there exists a controller that ensures that the resultant system trajectory satisfies the specification.
% Mathematically, 
% \begin{equation} \label{eqn:quad:viability_kernel}
% \viableset_{\sys} = \{x(0): \exists u(0), u(1), \ldots, u(H-1), \traj_{\sys} \models \spec \}. 
% \end{equation}
% If the system model in \eqref{eqn:quad:model} is known, there exist several methods in literature to compute the viability kernel \SBnote{cite some viability kernel computation papers}. 
% However, we are interested in the setting where the system dynamics are unknown and only its abstraction is available. 
% We use the dynamics of the abstraction and the distance bound between the system and the abstraction, $d$, to construct an under-approximation of $\viableset_{\sys}$, $\viableset_{\abs}(d)$, such that if the abstraction satisfies the specification with the augmented avoid set, $\spec(d)$, then the system must satisfy the actual specification. Here
% %
% \begin{align} \label{eqn:quad:approx_kernel}
% \viableset_{\abs}(d) = \{x(0): \exists u(0), u(1), \ldots, u(H-1), \traj_{\abs} \models \spec(d) \}, \nonumber \\
% \spec(d) = \forall t \in \{0, 1, \ldots, H\}, 0.5m + d \leq z(t) \leq 2.5m - d.
% \end{align}
% %

% Using a large enough distance bound $d$ can ensure that $\viableset_{\abs}(d) \subset \viableset_{\sys}$, and thus $\viableset_{\abs}(d)$ can be used as an under approximation of $\viableset_{\sys}$. 
% However, as $d$ increases the approximation gets more and more conservative. 
% Thus, the aim is to compute a $d$ such that $\viableset_{\abs}(d) \subset \viableset_{\sys}$, but $\viableset_{\sys} - \viableset_{\abs}(d)$ is small.
% We illustrate that the proposed distance metric in \eqref{eqn:mod_sim_metric} is able to capture these trade-off.

% Let's consider an abstraction with the same dynamics as in \eqref{eqn:quad:model}, except that the value of the parameter $k$ in the abstraction, $k_{\abs}$ is different.
% In particular, we consider two scenarios: $k_{\abs} < k$ and $k_{\abs} > k$.

==> sections/running_example_computation_old.tex <==
\section{Running Example: Distance Computation}
\label{Sec:example_distComp}
We now apply the proposed algorithm to design a safe controller for the system for the setting described in Section \ref{sec:running_example:description}.
For any given environmental scenario $\env$ (which essentially consists of a desired state $\state^*$), the space of controllers $\controlspace$ is given by
\begin{equation}
\controlspace_{\Pi} = \{LQR(q): 0.1 \leq q \leq 100\},
\end{equation}
where $LQR(q)$ is a Linear Quadratic Regulator (LQR) designed for the abstraction dynamics in \eqref{eqn:running_example:abs_dynamics} to regulate the abstraction trajectory to $\state^*$ \footnote{That is, we penalize the trajectory deviation to the desired state $\state^*$ in the LQR cost function.}, with the state penalty matrix $Q = qI$ and the control penalty coefficient $R = 1$.
Thus, for different values of $q$ we get different controllers, which affect the various characteristics of the resultant trajectory, such as overshoot, undershoot, final state, etc. 
$LQR(q)$ for any given $q$ can be obtained by solving the discrete-time Riccati equation~\cite{kwakernaak1972linear}.
The set of controllers $\controlspace_{\spec(\env)}$ and $\controlspace_{\spec(\env, \dist)}$ are then given as 
%
\begin{align} \label{eqn:running_example:prop_condition}
\controlspace_{\spec(\env)} = & \{\ctrlseq \in \controlspace_{\Pi}: \|\traj_{\sys}(\horizon; \state_0, \ctrlseq) - \state^*\|_2 < \gamma \}, \nonumber \\
\controlspace_{\spec(\env, \dist)} = & \{\ctrlseq \in \controlspace_{\Pi}: \|\traj_{\sys}(\horizon; \state_0, \ctrlseq) - \state^*\|_2 < \gamma - \dist \}.
\end{align}
%
Thus, we trivially have $\controlspace_{\spec(\env, \dist)} \subset \controlspace_{\spec(\env)}$ for any $\dist \geq 0$.

Note that we can very well use the set of all possible finite horizon control sequences for $\controlspace_{\Pi}$, but more often than not, a systematic process is used to design a controller to achieve the desired behavior. 
For example, to regulate a system to a desired state, LQR provides a much more efficient way of designing a controller compared to searching over all finite horizon control sequences. 
Moreover, the controller obtained through LQR is a state feedback controller that provides robustness to external disturbances.

To illustrate the utility of the different components in our distance metric, we compute four different distance metrics between $\sys$ and $\abs$:
\begin{enumerate}
    \item $\distMetricOld$ as in \eqref{eqn:sim_metric:naive};
    \item $\distMetricNew$ as in \eqref{eqn:sim_metric:proposed};
    \item $\distMetricIntOne$ defined as:
        \begin{equation}
        \label{eqn:sim_metric:naive2}
        \distMetricIntOne = \max_{\env \in \Env} \max_{u \in \controlspace_{\spec(\env)}} \|\traj_{\sys}(\cdot; \state_0, \ctrlseq) - \traj_{\abs}(\cdot; \state_0, \ctrlseq) \|_{\infty}, 
        \end{equation}
    \item $\distMetricIntTwo$ defined as:
        \begin{equation}
        \label{eqn:sim_metric:naive3}
        \distMetricIntTwo = \max_{\env \in \Env} \max_{u \in \controlspace_{\spec(\env)}} \|\traj_{\sys}(\cdot; \state_0, \ctrlseq) - \traj_{\abs}(\cdot; \state_0, \ctrlseq) \|_{\infty} \cdot \mathbbm{1}_{\left(\traj_{\sys}(\cdot) \not \models \spec(\env)\right)}, 
        \end{equation}
\end{enumerate}
\noindent where $\infty$-norm is the maximum distance between the trajectories across all timesteps and $\mathbbm{1}_l$ is the indicator function which is $1$ if $l$ is true and $0$ otherwise.
Note that the distance metric in \eqref{eqn:sim_metric:naive2} is same as $\distMetricOld$, except that the distance bound is computed over only those controllers that satisfy the specification for $\abs$, and not over all possible finite-horizon controllers. 
In distance metric $\distMetricIntTwo$ we further restrict the distance computation to the unsafe trajectories of $\sys$.
% ; however, still only those controllers that violate the specification on the system and satisfy it on the model contribute to the distance bound. 
We next compute $\distMetricNew$ using Algorithm \ref{alg:solution}, and the other three distance metrics using a modification of Algorithm \ref{alg:solution} where the corresponding distance function is used in Step4 instead.
For $\distMetricOld$, we sample a random control sequence over the horizon as opposed to sampling a feasible control sequence in Step2. 

According to the scenario approach with $\epsilon=0.01$ and $\beta=10^{-6}$, we extract $N=2964$ different environmental scenarios (i.e., $N$ different final states to reach.)
For each $\env_i, i \in \{1, 2, \ldots, 2964\}$, we obtain a feasible LQR controller $\ctrlseq_i \in \controlspace_{\spec(\env_i)}$ using rejection sampling. 
In particular, we randomly sample a penalty parameter $q$, solve the corresponding Riccati equation to obtain $LQR(q)$ and apply it on the model. 
If the model satisfies the specification, i.e., if the model trajectory is in the reach set at the final timestep, we use $\ctrlseq_i$ as our feasible controller sample; otherwise, we sample a new $q$ and repeat the procedure until a feasible controller is found.
This procedure tends to be really fast and requires a simulation only on the abstraction and not the system. 
For example, a feasible controller was found within 3 samples of $q$ for all $\env_i$ in this case.
For $\distMetricOld$, we randomly sample a control sequence for each $\env_i$, where control input at each timestep is uniformly sampled from $[-10, 10]$.

The corresponding distance metrics obtained are $\distMetricOld = 1.11, \distMetricIntOne = 0.43, \distMetricIntTwo = 0., \distMetricNew = 0.$
To synthesize a safe controller for $\sys$, we can now synthesize a controller for $\abs$ for the modified specification $\spec(\env; \dist)$, where $\dist$ is the corresponding distance metric.
In this case, the modified specification $\spec(\env; \dist)$ requires to contract the radius of the reach set to $(\gamma - \dist)$.
Since $\distMetricOld > \gamma$, there does not exist any controller that satisfies the modified specification $\spec(\env; \distMetricOld)$.
Consequently, we cannot synthesize a safe controller for the system for any environmental scenario using this distance metric, rendering it impractical for verification purposes. 
Since $\distMetricIntOne < \gamma$, it is still possible to synthesize a safe controller for $\sys$ using this distance metric, indicating the utility of restricting the controller search to the set of controllers that satisfy the specification for $\abs$. 
However, the controller still needs to satisfy a much tighter specification of reaching within a ball of radius 0.07 around the target state, which might significantly reduce the number of environmental scenarios for which we can synthesize a safe controller.
In contrast, $\distMetricIntTwo$ and $\distMetricNew$ are both zero. 
Since $\controlspace_{\spec(\env, \dist)} \subset \controlspace_{\spec(\env)}$ for any $\dist \geq 0$ (see \eqref{eqn:running_example:prop_condition}), Proposition \ref{prop:main_result_2} ensures that any controller designed on $\abs$ that satisfies the \textit{original} specification is guaranteed to satisfy the specification on $\sys$ as well.

Moreover, in this case, the dynamics of $\sys$ and $\abs$ are same for the state $\state_1$, and state $\state_2$ is uncontrollable for $\sys$ and remain $0$ at all times.
Thus, any controller that reaches within a ball of radius $\gamma$ around a desired state $\state_1^*$ for $\abs$, if applied on $\sys$, must also ensure that the system state reaches within the same ball.
Even though this information is unknown to all distance metrics, $\distMetricNew$ and $\distMetricIntTwo$ are able to capture it only through simulations on $\sys$, because only those controllers that satisfy the specification on $\abs$ but not on $\sys$ contribute to the distance metric, and no such controller exists in this case. 
This example illustrates that $\distMetricIntTwo$ and $\distMetricNew$ significantly reduce the conservativeness in the simulation metric. 
Note that in this case $\distMetricIntTwo$ and $\distMetricNew$ are equal, but that is not necessarily always the case.
$\distMetricNew$ further reduces the conservativeness in $\distMetricIntTwo$, as illustrated in Section \ref{sec:quadrotor}.

Further, $\Env_{\spec}(\distMetricOld) = \emptyset$ and  $\Env_{\spec}(\distMetricNew) = \Env_{\spec}$, illustrating that the unmodified simulation metric $\distMetricOld$ cannot be used to synthesize a safe controller for $\sys$ for any environmental scenario.

==> sections/solution_approach_old.tex <==
\section{Solution Approach}
\label{sec:approach}
\subsection{Generate approximate safe sets using $\abs$}
Computing sets $\Env_{\sys}$ and $\controlspace_{\sys}$ exactly can be quite challenging since the dynamics of $\sys$ are unknown apriori. 
Generally, we use the abstraction $\abs$ as a replacement for $\sys$ to synthesize safe controllers for $\sys$. 
However, to provide guarantees on $\sys$ using $\abs$, we would need to quantify how different the two are.
% Computing~\eqref{eqn:ideal_sets:1} and~\eqref{eqn:ideal_sets:2} exactly is not possible since $\sys$ is unknown apriori. To find $\env_{\sys}$ and $\controlspace_{\sys}$; for each $\env \in \Env$, we would have to exhaustively test every $\ctrlseq \in \controlscheme(\env)$ on the $\sys$. This is impractical. Generally, we use the abstraction $\abs$ as a replacement for the $\sys$ to synthesize safe controllers $\ctrlseq$ for the system. This $\abs$ is in general simpler and easier to analyze. However, to correctly analyze $\abs$ (and hence provide guarantees on $\sys$), we would need to quantify how different the two are. 
%We could approximate~\eqref{eqn:ideal_sets:1} by, 
%\begin{equation}
%\label{eqn:approx_sets:1}
%    \Env_{\spec} = \{\env \in \Env: \forall \ctrlseq \in \controlscheme(\env)\,, \traj_{\abs}(\cdot) \models \spec_{\env} \wedge \traj_{\sys}(\cdot) \models \spec_{\env} \}
%\end{equation}
%Within~\eqref{eqn:approx_sets:1}, the $\abs$ can be used instead of $\sys$ to synthesize safe controller. In $\Env_{\spec}$, whatever controller is safe for $\abs$is also safe for $\env$. This is the \textbf{largest} set of $\Env \subset \Env_{\sys}$, where the $\abs$ can be used to synthesize safe controllers for $\sys$. There is no systematic way to compute $\Env_{\spec}$, we would have to exhaustively go through each $\env, \ctrlseq \in \controlscheme(\env)$ pair to find the associated safe environments and controllers.

This bound, $\dist$, between $\sys$ and $\abs$ can then be used to approximate~\eqref{eqn:ideal_sets:1} and~\eqref{eqn:ideal_sets:2} using only $\abs$. 
$\dist$ is used to ``expand'' the avoid set $\avoidSet(\cdot)$ to get the augmented avoid set $\avoidSet(\cdot; \dist) = \avoidSet(\cdot) \oplus \dist$. Similarly, we can ``contract'' the $\reachSet(\cdot)$ with $\dist$ to obtain  a conservative reach set $\reachSet(\cdot; \dist) = \reachSet(\cdot) \ominus \dist$. Here, $\oplus$ ($\ominus$) are the Minkowski sum(difference). Consequently, the specification $\spec(\env)$ is modified to $\spec(\env; \dist)$. $\spec(\env; \dist)$ can be defined in a similar manner to $\spec(\env)$ to be the set of trajectories which avoid $\avoidSet(\cdot; \dist)$ and are always contained in $\reachSet(\cdot; \dist)$, 
\begin{equation}
    \label{eqn:spec:modified}
    \spec(\env; \dist) :=\{\traj(\cdot): \traj(t) \notin \avoidSet(t; \dist), \traj(t) \in \reachSet(t; \dist) \forall t \in \timeHorizon\}
\end{equation}$\dist$ is computed in such
Since $\dist$ quantifies the difference between $\abs$ and $\sys$ behavior; if $\abs$ to satisfies $\spec(\env;\dist)$, the system would satisfy $\spec(\env)$. Formally, $\forall \env \in \Env \, , \ctrlseq \in \controlscheme(\env) \, \traj_{\abs}(\cdot) \models \spec(\env; \dist) \rightarrow \traj_{\sys}(\cdot) \models \spec(\env)$.

\noindent For all $\env \in \Env$, we define the set of feasible of controllers for a modified specification $\spec(\env; d)$ as, 
\begin{equation}
\label{eqn:controller:modified}
    \begin{split}
        \controlspace_{\spec(\env; d)}  & :=\{\ctrlseq \in \controlscheme(\env): \traj_{\abs}(\cdot; \state_0, \ctrlseq) \models \spec(\env; d)\}\\
        & = \{\ctrlseq \in \controlscheme(\env): \traj_{\abs}(\time) \notin \avoidSet(\time; d) \wedge  \traj_{\abs}(\time) \in \reachSet(\time; d)\}
    \end{split}
\end{equation}
Hence, for each $\env \in \Env$\,, $\controlspace_{\spec(\env; d)}$ we have $\traj_{\abs}(\cdot) \models \spec(\env; \dist)$ and $\traj_{\sys}(\cdot) \models \spec(\env)$.

The set of safe environments can be defined as, 
\begin{equation}
\begin{split}
\label{eqn:equation:modified}
    \Env_{\spec}(d)& : = \{\env \in \Env: \exists \ctrlseq \in \controlscheme(\env) \, \traj_{\abs}(\cdot) \models \spec(\env; d)\} \\
    & = \{\env \in \Env: \controlspace_{\spec(\env, d)} \neq \emptyset\}\\
\end{split}
\end{equation}
$\Env_{\spec}(\dist)$, is the set of all environments for which there exists a controller that satisfies the modified specification $\spec(\env; \dist)$ for the abstraction; and hence $\spec(\env)$ for the system. We have reduced the problem of finding $\Env_{\sys}$ and $\controlspace_{\sys}$ using $\sys$ to computing the largest $\Env_{\spec}$ and $\controlspace_{\env}$ using the $\abs$. Thus, we would expect to see a large reduction in complexity. 
Specifically, the verification problem for the system 
\begin{equation*}
    \forall \env \in \Env_{\sys} \, \forall \ctrlseq \in \controlscheme(\env) : \traj_{\sys}(\cdot) \models \spec(\env) 
\end{equation*}
reduces to finding $\dist$, such that,
\begin{equation*}
\forall \env \in \Env_{\spec}(\dist) \, \forall \ctrlseq \in \controlspace_{\spec(\env; \dist)} : \traj(\abs) \models \spec(\env; \dist) \textit{and hence, } \traj_{\sys}(\cdot) \models \spec(\env)
\end{equation*}


We first show how $\dist$ can be computed using the simulation metric. However, the simulation metric as defined in literature, give us a conservative $\Env_{\spec}(\dist)$.
 We next introduce a new simulation metric which is less conservative and returns the \textbf{largest} $\Env_{\spec}(\dist) \subseteq \Env_{\sys}$ among all distance metrics. 

\subsection{Computing $\dist$ using Simulation Metric}
One way of computing $\dist$ is using the simulation metric.
%We first show how the simulation metric can be used to approximate $\Env_{\spec}$. However, the simulation metric as defined in literature, give us conservative estimates of $\Env_{\spec}$. We next introduce a new simulation metric which is less conservative and returns the largest $\Env_{\spec} \subseteq \tilde{\Env}_{\spec}$, i.e., computes the largest $\Env$ set where $\abs$ can provide strong safety guarantees for the $\sys$.

The simulation metric between $\abs$ and $\sys$ is defined as,
\begin{equation}
\label{eqn:sim_metric:naive}
    \distMetricOld = \max_{\env \in \Env} \max_{\ctrlseq \in \controlscheme(\env)} \|\traj_{\sys}(\cdot; \state_0, \ctrlseq) - \traj_{\abs}(\cdot; \state_0, \ctrlseq) \|_{\infty}
\end{equation}
%where $\controlspace$ is the set of all finite horizon controls over $\timeHorizon$ and $\traj_{\abs}$ ($\traj_{\sys}$) is the associated trajectory of the abstraction (system). 
Here, the $\infty$-norm is the maximum distance between the trajectories.
%Several methods have been proposed in literature to compute $\distMetricOld$, when $\sys$ is not available, using the data-driven methods.
\eqref{eqn:sim_metric:naive} computes the open-loop distance between the $\abs$ and $\sys$. Typically the simulation metric is defined over the space of all finite horizon controls $\controlspace$ instead of $\controlscheme(\env)$. When defined in the space of $\controlspace$, this distance is defined as approximate simulation metric~\cite{Girard2011}. Such a metric is difficult to compute, because it requires exhaustively searching over (the potentially infinite) space of $\controlspace$. An approximate technique was presented for systems whose dynamics were unknown with probabilistic guarantees in~\cite{Abate2011}.   
%\SBnote{Cite some simulation metric computation methods when a dynamics model of the system is not available. Also appreciate the fact that computation is not a very straightforward problem, and defer the discussion on the computation until the next section.}
% The $d(\cdot, \cdot)$ is generally 2-norm, although any $p$-norm can be considered. The 2-norm has the special property which guarantees that independent of the control sequence chosen, the resulting trajectories of the system and model are bounded by $d_N^*$.

%Once $\distMetricOld$ is obtained, we can ``expand'' the avoid set $\avoidSet(\cdot)$ with $\distMetricOld$ to get the augmented avoid set $\avoidSet(\cdot; \distMetricOld) = \avoidSet(\cdot) \oplus \distMetricOld$. Similarly, we can ``contract'' the $\reachSet(\cdot)$ with $\distMetricOld$ to obtain the a conservative reach set $\reachSet(\cdot; \distMetricOld) = \reachSet(\cdot) \ominus \distMetricOld$. Here, $\oplus$ ($\ominus$) are the Minkowski sum(difference). Since we modified the reach and avoid set, the specification $\spec(\env)$ has to be modified to $\spec(\env; \distMetricOld)$. $\spec(\env; \distMetricOld)$ can be defined in a similar manner to $\spec(\env)$ to be the set of trajectories which avoid $\avoidSet(\cdot; \distMetricOld)$ and are always contained in $\reachSet(\cdot; \distMetricOld)$, 
%
%\begin{equation} \label{eqn:problem:spec_modified}
% \spec(\env; \distMetricOld) := \forall \time \in \timeHorizon, \traj(\time) \notin \avoidSet(\time; \distMetricOld), \traj(\time) \in \reachSet(\time; \distMetricOld),
%\end{equation}

%
If we could compute $\distMetricOld$ exactly, it can be shown that, 
\begin{proposition} \label{prop1}
For any $\env \in \Env$ and controller $\ctrlseq \in \controlspace$, we have $\traj_{\abs}(\cdot; \state_0, \ctrlseq_{\env}) \models \spec(\env; \distMetricOld)$ implies $\traj_{\sys}(\cdot; \state_0, \ctrlseq_{\env}) \models \spec(\env)$.
\end{proposition}
\noindent The proof of Proposition \ref{prop1} can be found in Section~\ref{sec:appendix}.
Proposition \ref{prop1} states that all the controllers that are safe for the abstraction with the modified specification are provably safe for the system with the original specification. However, if a controller is not safe for the abstraction, it may or may not be safe for the system.

%Since $\distMetricOld$ is computed using $\controlspace$ and not limited to $\controlscheme(\env)$; there is no systematic way of computing $\controlspace_{\spec(\env; \distMetricOld)}$.
%Given the difficulty in computing $\controlspace_{\spec(\env; \distMetricOld)}$, computing $\Env_{\spec}(\distMetricOld)$ is just as hard. 
%Given the difficulty in computing $\controlspace_{\spec(\env; \distMetricOld)}$, the best way to approximate $\Env_{\spec}(\distMetricOld)$, is 
%\begin{equation*}
%    \Env_{\spec}(\distMetricOld) := \{\env \in \Env: \forall \ctrlseq \in \controlspace\, , \traj_{\abs}(\cdot) \models \spec_{\env}(\distMetricOld) \}
%\end{equation*}
The sets $\controlspace_{\spec(\env; \distMetricOld)}$ and $\Env_{\spec}(\distMetricOld)$ can be defined appropriately. 
From Proposition~\ref{prop1}, for any $\env \in \Env_{\spec}(\distMetricOld)$, any $\controlspace_{\spec(\env; \distMetricOld)}$ is a safe controller for $\sys$, since it satisfies the modified specification on $\abs$.
%this is just an approximation of true $\Env_{\spec}(\distMetricOld)$, for which we would need to find that exact $\controlspace_{\spec(\env; \distMetricOld)}$ for each $\env \in \Env$.
% $\ctrlseq_{\env}$ is a provably safe controller for the system. 

The distance bound in~\eqref{eqn:sim_metric:naive} does not take into account the specification (environment) for which a controller needs to be synthesized. 
Thus, $\distMetricOld$ can be quite conservative. 
As a result, the avoid sets will be bigger and the reach sets will be smaller, and the set of environments $\Env_{\spec}(\distMetricOld)$ for which we can synthesize a provably safe controller for the abstraction (and hence for the system) itself will be very small.
%Moreover, $\distMetricOld$ considers $\controlspace$ to be the space of \textbf{all} controllers, w. 

\subsection{Proposed metric}
To overcome these limitations, we propose a modified simulation metric,
% However, considering~\eqref{eqn:sim_metric}, can be overly conservative. In general the purpose of the model is to synthesize controllers to perform a task $\param \in \paramspace$, using a specific control scheme $\Pi$ while satisfying certain high level safety specifications $\spec$. The $\spec$ should take into account the task $\param$ as well. These considerations reduce the set of controls we are likely to deploy on the system. Let us denote this set by $U \subset \controlspace$.
% In light of these factors, we propose a modified simulation metric, 
% \begin{equation}
% \label{eqn:sim_metric:proposed}
%     d^* = \max_{\param \in \paramspace} \max_{u \in \Pi(\param)} d(\traj_{\abs}, \traj_{\sys}) \mathbb{I}(\spec_{\abs}) \mathbb{I}(\neg \spec_{\sys})
% \end{equation}
% %
% \begin{equation}
% \label{eqn:sim_metric:proposed}
%     \distMetricNew = \max_{\env \in \Env} \max_{u \in \controlspace_{\spec(\env)}} \min_{\time \in \timeHorizon_{\spec(\env)}} \|\pos\left(\traj_{\sys}(\time; \state_0, \ctrlseq) - \traj_{\abs}(\time; \state_0, \ctrlseq)\right)\|,
% \end{equation}
% %
%
\begin{equation}
\label{eqn:sim_metric:proposed}
    \distMetricNew = \max_{\env \in \Env} \max_{u \in \controlspace_{\spec(\env)}}
    \dist(\traj_{\sys}(\cdot),\traj_{\abs}(\cdot)),
\end{equation}
%
where
%
\begin{equation}
    \label{eqn:dist_fn:proposed}
\begin{split}
    \dist(\traj_{\sys}(\cdot), \traj_{\abs}(\cdot)) = (\min_{\time \in \timeHorizon}
    (\min\{& \signdist\left(\traj_{\sys}(\time; \state_0, \ctrlseq), \avoidSet(\time)\right), \\ &
    -\signdist\left(\traj_{\sys}(\time; \state_0, \ctrlseq), \reachSet(\time)\right)
    \}) \mathbbm{1}_{\left(\traj_{\sys}(\cdot) \not\models \spec(\env)\right)}
    )
\end{split}
\end{equation}
%
Here $\controlspace_{\spec(\env)}:= \{\ctrlseq \in \controlspace_{\Pi}: \traj_{\abs}(\cdot; \state_0, \ctrlseq) \models \spec(\env)\}$ is the set of all controls such that, the abstraction satisfies the specification $\spec(\env)$.
%
%\begin{equation}
%\label{eqn:sim_metric:valid_ctrl}
%    \controlspace_{\spec(\env)} := \{\ctrlseq \in \controlspace_{\Pi}: \traj_{\abs}(\cdot; \state_0, \ctrlseq) \models \spec(\env)\},
%\end{equation}
%
$\mathbbm{1}_l$ represents the indicator function which is $1$ if $l$ is true and $0$ otherwise, 
and $\signdist(\state, K)$ is the signed distance function defined as
%
\begin{equation}
\label{eqn:sim_metric:sign_dist_func}
    \signdist(\state, K) := 
\begin{cases}
    \inf_{k \in K} \|\state - k\|, & \text{if } x\not\in K\\
    -\inf_{k \in K^C} \|\state - k\|, & \text{otherwise}
\end{cases}
\end{equation}
%
\noindent If for a $\env \in \Env$, $\controlspace_{\spec(\env)}$ is $\emptyset$, we define the distance function $\dist(\traj_{\sys}(\cdot), \traj_{\abs}(\cdot))$ to be zero since there does not exist a satisfying controller for the abstraction. 
Similarly, if there is no $\avoidSet$ or $\reachSet$ at a particular $\time$, the corresponding signed distance function is defined $\infty$.
% $\timeHorizon_{\spec(\env)}$ is the set of all times for which the system \textit{does not} satisfy the specification
% %
% \begin{equation}
% \label{eqn:sim_metric:valid_times}
%     \timeHorizon_{\spec(\env)} := \{\time \in \timeHorizon: \traj_{\sys}(\time; \state_0, \ctrlseq) \not\models \spec_{\time}(\env)\},
% \end{equation}
% %
% and $\pos(\cdot)$ are the components of the state $\traj(\cdot)$ that affect the specification.
% If for a $\env \in \Env$ and $\ctrlseq \in \controlspace_{\spec(\env)}$, $\timeHorizon_{\spec(\env)}$ is the $\emptyset$, then $\traj_{\sys}(\cdot) \models \spec_{\env}$, and $\dist(\traj_{\sys}, \traj_{\abs})$  evaluates to $0$.
% \SBnote{It would be good to give an example of $\pos$ for the running example here.}

There are four major differences between \eqref{eqn:sim_metric:naive} and \eqref{eqn:sim_metric:proposed}:
\begin{enumerate}
    \item To compute the distance bound we only consider the feasible set of controllers that can be synthesized by the control policy, $\controlspace_{\spec(\env)} \subseteq \controlscheme(\env)$, as all other controllers do not help us in synthesizing a safe controller for the system (as they are not even safe for the abstraction).
    \item To compute the distance between $\sys$ and $\abs$, we only consider those trajectories where the system violates the specification. 
    This is because a non-zero distance between the trajectories of $\sys$ and $\abs$, where the $\traj_{\sys} \models \spec(\env)$ does not give us any meaningful information.
    \item Within a falsifying $\traj_{\sys}$, we compute the minimum distance of the abstraction trajectory from the avoid sets rather than the system trajectory, as that is sufficient to obtain a margin to discard behaviors that are safe for the abstraction but unsafe for the system.
    \item Finally, a minimum over time of this distance is sufficient to discard an unsafe trajectory, as the trajectory will be unsafe if it is unsafe at any $\time$.
    % \item We only consider the states of the system that affect the specification using $g(\cdot)$.
    %\item to compute the distance bound we only consider the part of the trajectory where the system violates the specification; as any controller that ensures the system achieves our end goal, even though there is a non-zero distance between the trajectories of the system and the abstraction for that controller. 
    %Moreover, we only compute the minimum distance between the system and the model over such time points, because that is sufficient to capture if a controller ever violates the specification on the system;
\end{enumerate}
\noindent These considerations ensure that the proposed distance metric is far less conservative compared to the simulation metric in \eqref{eqn:sim_metric:naive} and allows us to synthesize a safe controller for the system for a wider set of environments.
%Ideally, we want to compute set $\Env_{\spec}$ and the corresponding set of safe controllers, but its direct computation is non-trivial.
%Instead, we compute a distance bound $d$ between $\sys$ and $\abs$ such that $\Env_{\spec}(\dist) \subset \Env_{\spec}$; $\Env_{\spec}(\dist)$ is then used as a conservative approximation of $\Env_{\spec}$.
%However, the size of the set $\Env_{\spec}(\dist)$ depends on the different distance metrics. One way to measure the utility of a distance metric is through the size of the set $\Env_{\spec}(\dist)$; because we can synthesize a safe controllers for $\sys$ using $\abs$ for the environment scenarios in $\Env_{\spec}(\dist)$.
%Ideally, the distance metric should be such that $\Env_{\spec}(\dist)$ is as large as possible, while still ensuring $\Env_{\spec}(\dist) \subseteq \Env_{\spec}$ (ideally $= \Env_{\spec}$.)

%
\noindent We can do
\begin{proposition} \label{prop:main_result_1}
Let $\distMetricNew$ be defined as in \eqref{eqn:sim_metric:proposed}.
If $\controlspace_{\spec(\env, \distMetricNew)} \subseteq \controlspace_{\spec(\env)}$, then $\traj_{\abs}(\cdot; \state_0, \ctrlseq_{\env}) \models \spec(\env; \distMetricNew)$ implies $\traj_{\sys}(\cdot; \state_0, \ctrlseq_{\env}) \models \spec(\env)$.
\end{proposition} 
%
\noindent The proof of Proposition \ref{prop:main_result_1} can be found in Section~\ref{sec:appendix}. 
%Intuitively, to compute~\eqref{eqn:sim_metric:proposed}, we only consider $\traj_{\abs}, \traj_{\sys}$ where $\traj_{\abs}\models \spec(\env)$ but $\traj_{\sys} \not\models \spec(\env)$.~\eqref{eqn:sim_metric:valid_times} ensures that we only consider the part of the trajectory where $\traj_{\sys}$ falsifies the specification. 
Intuitively, $\distMetricNew$ is the smallest distance which guarantees that any feasible safe controller for $\abs$ is safe for the $\sys$. 
This is because, to compute $\distMetricNew$, we only consider the controllers that are safe for $\abs$ but unsafe for $\sys$. 
Specifically, for each such $\ctrlseq$, we compute the minimum distance which will render this controller unsafe for $\abs$. 
% This is guaranteed by~\eqref{eqn:dist_fn:proposed}. 
Hence, expanding $\avoidSet$ and contracting $\reachSet$ by the maximum of this distance across all $\ctrlseq \in \controlspace_{\spec(\env)}$, i.e. $\distMetricNew$, guarantees we have refuted each $\ctrlseq$ that is safe for $\abs$ but unsafe for $\sys$. 
This ensures that there does not exist a $\traj_{\sys}$ that falsifies $\spec(\env)$ if the $\traj_{\abs}$ satisfies the modified specification, $\spec(\env;\distMetricNew)$.
Thus, a safe controller for $\abs$ for the modified specification is provably safe for $\sys$. 

$\Env_{\spec}(\distMetricNew)$ is the set of environments where the set of $\controlspace_{\spec(\env, \distMetricNew)} \neq \emptyset$. $\controlspace_{\spec(\env, \distMetricNew)}$ is the set of controllers which are safe for the $\abs$ for the modified specification $\spec(\env; \distMetricNew)$ and hence safe for $\sys$. As long as this is not empty for an $\env \in \Env$, we can safely guarantee that a safe controller for $\sys$ exists for such an environment. 

% Proposition \ref{prop:main_result_1} ensures that the distance bound computed in \eqref{eqn:sim_metric:proposed} is sufficient to design a safe controller for the system.
Note that Proposition \ref{prop:main_result_1} requires that the set of controllers $\controlspace_{\spec(\env, \distMetricNew)}$ that satisfy the modified specification be a subset of the set of the controllers $\controlspace_{\spec(\env)}$ that satisfy the actual specification. 
This is to ensure that the distance bound computation has taken into account all controllers that are potential candidates during test time. 

%\begin{remark} \label{rem:control_containment}
%It is easy to see, that for any $\ctrlseq \in \controlspace_{\Pi}$, we have $\traj_{\abs}(\cdot; \state_0, \ctrlseq) \models \spec(\env; d) \rightarrow \traj_{\abs}(\cdot; \state_0, \ctrlseq) \models \spec(\env)$; since $\spec(\env; d)$ guarantees that the $\traj_{\abs}(\cdot)$ is at least $d$ distance away from $\avoidSet(\cdot)$ (and $\reachSet(\cdot)$) at all times. 
%Hence, we have $\controlspace_{\spec(\env; d)} \subseteq \controlspace_{\spec(\env)}$. 

%Following the above reasoning we have, if $d < d'$ then $\controlspace_{\spec(\env; d')} \subseteq \controlspace_{\spec(\env; d)}$.
%\end{remark}

\begin{remark}\label{rem:control_containment}
If for any $d \in \reals$, we have $\controlspace_{\spec(\env; d)} \subset \controlspace_{\spec(\env)}$; then for any $d ,d'$ such that $d < d'$ we have $\controlspace_{\spec(\env; d')} \subset \controlspace_{\spec(\env; d)}$. 

The space $\controlspace_{\spec(\env; d)}$ is a total order in $d$.
\end{remark}

When $\controlspace_{\Pi}=\controlspace$, this condition is trivially satisfied as the modified specification is more stringent than the actual specification. 
%From Remark~\ref{rem:control_containment}, we have this always holds true when we consider the the controllers are synthesized by a control scheme $\Pi$.
However, Proposition \ref{prop:main_result_1} also holds when $\controlspace$ is limited to the set of controllers generated by a particular scheme, e.g. linear feedback controllers, in which case this condition needs to be explicitly ensured. 

Remark~\ref{rem:control_containment} is not a very restrictive constraint on the control policies that can be considered for distance metric. In general, feedback controllers (e.g. Linear Quadratic regulators), feasible set controllers returned by optimization (e.g. all feasible Model Predictive controllers), reachability based control sets satisfies Remark~\ref{rem:control_containment}. However, if we only consider the optimal controllers returned by optimization techniques, Remark~\ref{rem:control_containment} does not hold; since we do not have set of all feasible controllers.

\begin{remark}
We have for $d < d'$, the set $\Env_{\spec}(d') \subseteq \Env_{\spec}(d)$ since $\forall \env \in \Env$, the set of feasible controllers $\controlspace_{\spec(\env; d)} \subseteq \controlspace_{\spec(\env; d')}$ (from Remark~\ref{rem:control_containment}).
\end{remark}

The proposed distance metric $\distMetricNew$ allows us to verify the system for all environmental scenarios that are verifiable using the abstraction when the system dynamics are perfectly known.
%In fact, it can be proved that is the case whenever $\abs$ is a conservative approximation of $\sys$.
%
%\begin{proposition} \label{prop:main_result_3}
%Let $\abs$ and $\sys$ be such that $\forall \env \in \Env\; \forall \ctrlseq \in \controlscheme(\env)$\; $\traj_{\abs}(\cdot; \state_0, \ctrlseq) \models \spec(\env)$ implies $\traj_{\sys}(\cdot; \state_0, \ctrlseq) \models \spec(\env)$. Then, $\distMetricNew = 0$ and $\Env_{\spec}(\distMetricNew) = \Env_{\sys}$.
%\end{proposition}
%

%Intuitively, Proposition \ref{prop:main_result_3} claims that whenever $\abs$ is a conservative approximation of  $\sys$; i.e. the safe behaviors of $\abs$ is a subset of the safe behaviors of $\sys$; the proposed distance metric will be able to recover the verifiable set $\Env_{\sys}$ exactly.
%This is interesting because the proposed metric is able to do so without knowing that $\abs$ is a conservative approximation of $\sys$ beforehand.
%$\distMetricNew$ evaluates to $0$, even without knowing apriori that the condition holds.
%Note that this is not necessarily the case for the distance metrics $\distMetricOld$, indicating its conservative nature as far as the specification satisfaction is concerned.

%However, if $\abs$ is not a conservative approximation of $\sys$, then $\distMetricNew \neq 0$, as it should be. 
Our metric, $\distMetricNew$, quantifies the tightest (largest) approximation of $\Env_{\sys}$, i.e., $\nexists d < \distMetricNew$, such that $\Env_{\spec}(d) \subseteq \Env_{\sys}$. 
%In such cases, our goal is still to obtain the best possible approximation of $\Env_{\spec}$ and the proposed distance metric still outperforms the other three distance metrics, as illustrated in Section \ref{sec:case_studies}.

\begin{theorem}
\label{thm:min_dist}
The solution to~\eqref{eqn:sim_metric:proposed}, $\distMetricNew$, ensures that, 
\begin{enumerate}
    \item $\spec(\env; \distMetricNew)$ is the tightest specification that guarantees Proposition~\ref{prop:main_result_1}.
    \item $\Env_{\spec}(\distMetricNew)$ is the tightest (largest) set of feasible environments where if there exists a controller for the $\abs$ it is safe for $\sys$. Hence, $\Env_{\spec}(\distMetricNew)$ quantifies the tightest (largest) approximation of $\Env_{\sys}$.
    \item $\controlspace_{\spec(\env; \distMetricNew)} \in \controlscheme(\env)$ is the largest set of safe controllers for $\sys$; i.e., $ \forall \ctrlseq \in \controlspace_{\spec(\env; \distMetricNew)} \traj_{\sys} \models \spec(\env)$ in any $\env  \in \Env_{\spec}(\distMetricNew)$.
\end{enumerate}
\end{theorem}

The proof for Theorem~\ref{thm:min_dist} can be found in the appendix. Intuitively statement (1)-(3) in Theorem~\ref{thm:min_dist} follows if we can prove there $\nexists d < \distMetricNew$ that for any $\env \in \Env$; refutes all $\ctrlseq \in \controlspace_{\spec(\env)}$ where $\traj_{\abs}(\cdot) \models \spec(\env)$ but $\traj_{\sys}(\cdot) \not\models \spec(\env)$. 
Intuitively, one can imagine to compute~\eqref{eqn:sim_metric:proposed}, we collect all $\traj_{\abs}(\cdot), \traj_{\sys}(\cdot)$ pair (across all $\env \in \Env$ and $\ctrlseq \in \controlspace_{\spec(\env)}$) where $\traj_{\abs}(\cdot) \models \spec(\env)$ and $\traj_{\sys}(\cdot) \not\models \spec(\env)$. 
We then evaluate~\eqref{eqn:dist_fn:proposed} for each pair and take the maximum value to compute $\distMetricNew$. By expanding (contracting) any $\avoidSet \in \avoidSets$ ($\reachSet \in\reachSets$) uniformly by $\distMetricNew$, we ensure that none of the $\traj_{\abs}(\cdot)$ collected above can occur during test-time and hence, $\traj_{\sys}(\cdot)$ will never falsify $\spec(\env)$.   


